Automatic Generation of Contrast Sets from Scene Graphs: Probing the Compositional Consistency of GQA

Recent works have shown that supervised models often exploit data artifacts to achieve good test scores while their performance severely degrades on samples outside their training distribution. Contrast sets (Gardneret al., 2020) quantify this phenomenon by perturbing test samples in a minimal way such that the output label is modified. While most contrast sets were created manually, requiring intensive annotation effort, we present a novel method which leverages rich semantic input representation to automatically generate contrast sets for the visual question answering task. Our method computes the answer of perturbed questions, thus vastly reducing annotation cost and enabling thorough evaluation of models' performance on various semantic aspects (e.g., spatial or relational reasoning). We demonstrate the effectiveness of our approach on the GQA dataset and its semantic scene graph image representation. We find that, despite GQA's compositionality and carefully balanced label distribution, two high-performing models drop 13-17% in accuracy compared to the original test set. Finally, we show that our automatic perturbation can be applied to the training set to mitigate the degradation in performance, opening the door to more robust models.

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/figs/breakdown.tex <==
\begin{table}[tb!]
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
                                                        & \multicolumn{2}{c}{\textbf{MAC}}                                               & \multicolumn{2}{c}{\textbf{LXMERT}}                                            \\ \midrule
                                                        & \multicolumn{1}{c}{\textbf{Original}} & \multicolumn{1}{c}{\textbf{Aug.}} & \multicolumn{1}{c}{\textbf{Original}} & \multicolumn{1}{c}{\textbf{Aug.}} \\
\text{On which side is the \textbf{\textit{X}}?}                    & 68\%                                  & 57\%                                   & 94\%                                  & 81\%                                   \\
\text{What color is the \textbf{\textit{X}}?}                        & 49\%                                  & 49\%                                   & 69\%                                  & 62\%                                   \\
\text{Are there \textbf{\textit{X}} near the \textit{Y}?}                    & 85\%                                  & 66\%                                   & 98\%                                  & 79\%                                   \\
\text{Do you see \textbf{\textit{X}} or \textbf{\textit{Y}}?}                         & 88\%                                  & 53\%                                   & 95\%                                  & 65\%                                   \\
\text{Is the \textbf{\textit{X}} \textit{Rel} the \textit{Y}?}        & 85\%                                  & 44\%                                   & 96\%                                  & 69\%                                   \\
\text{Is the \textit{X} \textbf{\textit{Rel}} the \textit{Y}?} & 71\%                                  & 38\%                                   & 93\%                                  & 55\%                                   \\
\text{Overall}                                        & 65\%                                  & 52\%                                   & 84\%                                  & 67\%                                   \\ \bottomrule
\end{tabular}
}
\caption{Model accuracy on the original and augmented validation set by question template for a maximum 5 augmentations per instance. }
\label{tab:results_single_augmentation}
\end{table}

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/figs/question_templates_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Question template}                              & \textbf{Tested attributes}           & \textbf{Example}                                                                                             \\ \midrule
On which side is the \emph{\textbf{X}}?                 & Relational (left vs.~right)          & On which side is the \textbf{\emph{dishwasher}}? $\rightarrow$ On which side are the \textbf{\emph{dishes}}?                   \\\midrule
What color is the \textbf{\textit{X}}?                  & Color identification                 & What color is the \textbf{\emph{cat}}?$\rightarrow$ What color is the \textbf{\emph{jacket}}?                                  \\\midrule
Do you see \textbf{\textit{X}} or \textbf{\textit{Y}}?  & Compositions                     & Do you see \textbf{\emph{laptops}} or cameras?$\rightarrow$ Do you see \textbf{\emph{headphones}} or cameras?            \\ \midrule
Are there \textbf{\textit{X}} near the \textit{Y}?      & \multirow{3}{*}{Spatial, relational} & Are\resolved{\emph{Are}\roy{why is the word ``Are'' in italics? I see that it changes to ``Is'' in the example, but this is confusing as you use italics to mark variables and this is not a variable}} there any \textbf{\emph{cats}} near the boat? $\rightarrow$ \emph{Is} there any \textbf{\emph{bush}} near the boat? \\
Is the \textit{X} \textbf{\textit{Rel}} the \textit{Y}? &                                      & Is the boy to the \textbf{\emph{right}} of the man? $\rightarrow$ Is the boy to the \textbf{\emph{left}} of the man?           \\
Is the \textbf{\textit{X}} \textit{Rel} the \textit{Y}? &                                      & \resolved{\roy{shouldn't Y be bold and not X in this line?}} Is the \textbf{\emph{boy}} to the right of the man? $\rightarrow$ Is the \textbf{\emph{zebra}} to the right of the man?        \\ \bottomrule
\end{tabular}%
}
\caption{Question templates with original question examples, and generated perturbations modifying the answer. Italic text indicates variables, bold text indicates the perturbed atoms.\resolved{\roy{minor: given that we mark perturbed atoms in bold in the template, can we do the same for the example (i.e., instead of italics?)}}}
\label{tab:question_templates}
\end{table*}

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/figs/results_table.tex <==
\begin{table}[t!]
\centering
\scalebox{0.90}{
\begin{tabular}{@{}lrcc@{}}
\toprule
\textbf{Model}            & \textbf{Training set}       & \textbf{Original} & \textbf{Augmented} \\ \midrule
\multirow{2}{*}{MAC}      & Baseline                        & 64.9\%            & 51.5\%             \\
                          & Augmented     & 64.4\%            & 68.4\%             \\ \midrule
\multirow{2}{*}{LXMERT}   & Baseline                        & 83.9\%            & 67.2\%             \\
                          & Augmented    & 82.6\%            & 77.2\%             \\
                          \bottomrule
\end{tabular}
}
\caption{Model accuracy on the original validation set and on our generated contrast sets with maximum of 5 augmentations.
\textit{Baseline} refers to the original models, \textit{augmented} refers to the models trained with our augmented  training contrast sets.\resolved{\roy{is this with 5 augmentations? 1? please add here and on the referring text}}}
\label{tab:training_improvement}
\end{table}

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/00_abstract.tex <==
Recent works have shown that supervised models often exploit data artifacts to achieve good test scores while their performance severely degrades on samples outside their training distribution.
\textit{Contrast sets} \cite{gardner-etal-2020-evaluating} quantify this phenomenon by perturbing test samples in a minimal way such that the output label is modified.  
While most contrast sets were created manually, requiring intensive annotation effort, we present a novel method which leverages rich semantic input representation to \emph{automatically} generate contrast sets for the visual question answering task. Our method computes the answer of perturbed questions, thus vastly reducing annotation cost and enabling thorough evaluation of models' performance on various semantic aspects (e.g., spatial or relational reasoning). We demonstrate the effectiveness of our approach on the popular GQA dataset \cite{hudson2019gqa} and its semantic scene graph image representation.
We find that, despite GQA's compositionality and carefully balanced label distribution, two strong models drop 13--17\%\resolved{\roy{use a long hyphen (-- and not -) when using numeric ranges}} in accuracy on our automatically-constructed contrast set compared to the original validation set.
Finally, we show that our method can be applied to the \emph{training} set to mitigate the degradation in performance, opening the door to more robust models.\footnote{Our contrast sets and code are available at \url{https://github.com/yonatanbitton/AutoGenOfContrastSetsFromSceneGraphs}.}

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/01_introduction.tex <==
\begin{figure}[!ht]
\centering
\newcommand{\figlen}[0]{\columnwidth}
    \includegraphics[width=\figlen]{images/example_figure1_with_table.png}\\%
    \includegraphics[width=\figlen]{images/scene_graph.png}

  \caption{
  %\roy{text is unreadable. can you please make it bigger?}
  Illustration of our approach based on an example from the GQA dataset. Top: QA pairs and an image annotated with bounding boxes from the scene graph. Bottom: relations among the objects in the scene graph. 
  First line at the top is the original QA pair, while  the following 3 lines show our \textit{pertubated} questions: replacing a single element in the question (\textit{a fence}) with other options (\textit{a wall, men, an elephant}), leading to  a change in the output label. 
  For each QA pair, the LXMERT predicted output is shown.
  }
    \label{fig:perturbed-example}
\end{figure}
NLP benchmarks typically evaluate in-distribution generalization, where test sets are drawn \textit{i.i.d} from a distribution similar to the training set. Recent works showed that high performance on test sets sampled in this manner is often achieved by exploiting systematic gaps, annotation artifacts, lexical cues and other heuristics, rather than learning meaningful task-related signal. As a result, the out-of-domain performance of these models is often severely deteriorated~\cite{jia-liang-2017-adversarial,ribeiro-etal-2018-semantically,gururangan-etal-2018-annotation, geva-etal-2019-modeling, mccoy-etal-2019-right, feng-etal-2019-misleading, stanovsky-etal-2019-evaluating}.
Recently, \citet{kaushik2019learning} and \citet{gardner-etal-2020-evaluating} introduced\com{(2) For the NLVR2 VQA variant \cite{suhr2019nlvr2} and other non VQA tasks,} the \textit{contrast sets} approach to probe out-of-domain generalization. Contrast sets are constructed via  minimal modifications to  test inputs, such that their label is modified. For example, in Fig.~\ref{fig:perturbed-example}, replacing ``a fence'' with ``a wall'', changes the answer from ``Yes'' to ``No''. Since such perturbations introduce minimal additional semantic complexity, robust models are expected to perform similarly on the test and contrast sets. However, a range of NLP models\com{including VQA datasets such as NLVR2 \cite{suhr2019nlvr2}, } severely degrade in performance on contrast sets, hinting that they do not generalize well~\cite{gardner-etal-2020-evaluating}. \com{(e.g., the answer to a ``Is there'' question is more often ``yes'' than ``no'' rather than more meaningful task signal)}Except two recent exceptions for textual datasets~\cite{li-etal-2020-linguistically, rosenman-etal-2020-exposing}, contrast sets have so far been built manually, requiring extensive human effort and expertise. %\footnote{Two concurrent works introduced automatic construction of contrast sets for text only tasks (NLI and relation extraction)~\citep{li-etal-2020-linguistically, rosenman-etal-2020-exposing}.}

%% ME: in reply to Roy's point at the beginning of next section,
%% I am adding here background on GQA as one way to address lack of compositionality in VQA and then on contrast sets.
%% This gives a full page before we explain what we do 
\com{To mitigate these biases,
several visual question answering (VQA) works constructed \textit{more balanced datasets}: 
most notably, \citet{goyal2017making} designed VQA V2, where the original VQA dataset is balanced such that every question is associated with a pair of similar images that result in two different answers to the question.
\citet{hudson2019gqa}\roy{When a citation is used as an entity in the sentence (
e.g., subject or object), cite it with citet and not cite}addressed the observed lack of generalization by designing GQA, a large-scale dataset of compositional questions over real-world images, starting from images from the Visual Genome, and ``leveraging semantic representations of both the scenes and questions to mitigate language priors and conditional biases and enable fine-grained diagnosis for different question types''.\roy{Is this a quote from the GQA paper? if so, put in italics and cite the paper again.} 
}


%% @@ME: The task of automatic contrast set construction has already been introduced in LIT - we need a rephrase to ack this
In this work, we propose a method for \emph{automatic} generation of large contrast sets for visual question answering (VQA). We experiment with the GQA dataset~\cite{hudson2019gqa}\resolved{\roy{this paper is cited twice, once 2018 and the other 2019}}. 
GQA includes semantic scene graphs~\cite{krishna2017visual} representing the spatial relations between objects in the image, as exemplified in Fig.~\ref{fig:perturbed-example}.
The scene graphs, along with functional programs that represent the questions, are used to \textit{balance} the dataset, thus aiming to mitigate spurious dataset correlations.
We leverage the GQA scene graphs to create contrast sets, by automatically computing the answers to question perturbations, e.g., verifying that there is no wall near the puddle in Fig.~\ref{fig:perturbed-example}.

% For example, for the \emph{perturbed question} in Fig.~\ref{fig:perturbed-example} we can automatically deduce from the scene graph that replacing ``a fence'' with ``a wall'' will change the gold answer from ``yes'' to ``no''. 
% We operationalize these observations to create contrast sets testing specific model capabilities, such as relative spatial reasoning or color identification. 

We create automatic contrast sets for 29K samples or $\approx$22\% of the validation set. We manually verify the correctness of 1,106 of these samples on Mechanical Turk.
Following, we evaluate two leading models, LXMERT \cite{tan-bansal-2019-lxmert} and MAC \cite{hudson2019gqa} on our contrast sets, and find a 13--17\%\resolved{\roy{use -- (see abstract comment)}} reduction in performance \com{(MAC from 64.9 to 51.5, LXMERT from 83.9 to 67.2)}compared to the original validation set. 
%% ME: Let's drop the explanation - we could not find a convincing one
%%We analyze our results, exploring the reasons for the drop in performance, and observe that models struggle with contrast questions containing objects not observed in the original training set.\roy{Yonatan please check} \yonatna{As we discussed - It's a weak correlation, I wouldn't mention the reason (Same as Gardner's paper - they don't explain)} \resolved{\roy{What are our main findings?} \yonatan{We hypothesize that we introduce "less-familiar" objects to the model. But it doesn't fully explain the performance gap, and leaves an open question. } }
Finally, we show that our automatic method for contrast set construction can be used to improve performance by employing it during \emph{training}.
We augment the GQA training set with automatically constructed  \emph{training contrast sets} (adding 80K samples to the existing 943K in GQA), and observe that when trained with it, both LXMERT and MAC improve by about $14\%$ on the contrast sets, while maintaining their original validation performance.

% (Altough the quality of the pertubations can be effected from the generation accuracy).

% \yonatan{Important addition, 
% Needs to be expressed better: } \textbf{Extending to other datasets}: Our method can be extended to other visual question answering datasets. If the dataset has information of the objects in the image such as scene graphs, we can perform the same augmentations. If the dataset doesn't have any kind of information, there is an option to use scene-graph predictions methods to obtain information about the image objects, and then perform the augmentation. 

Our key contributions are:
(1) We present an automatic method for creating contrast sets for VQA datasets with structured input representations;
(2) We automatically create contrast sets for GQA, and find that for two strong models, performance on the contrast sets is \resolved{significantly\roy{only use significantly if you computed statistical significance. Use ``substantially'' instead}}lower than on the original validation set; and
(3) We apply our method to augment the training data, improving both models' performance on the contrast sets.


==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/02_automatic.tex <==
\input{figs/question_templates_table}
%% ME - added background in intro
%% \roy{this is a short paper, so we don't have much room and are not expected to give tons of background, but at the same time I am missing background about both GQA and contrast sets. In particular, I don't think we say explicitly that GQA was constructed in a way that supposedly controls for data distribution, and is supposedly immune to artifacts. This might fit as a sentence or two in the intro but needs to be said explicitly. Second, you talk later about the \textit{contrast set approach}. What is this approach? just replacing minimal input in the document to change the label? or is there more to say about the approach?}
%%\yonatan{For the last question - yes, this approach is exactly as you said. Minimally changing the input such the answer is changed. Choosing 1 atom to change. I tried to do sophisticated modifications, such replace X with X' that is correlated with Y in some places, or replacing X with X' that is the most string-similar to X, etc. There can be much more ways to perform those modifications in a smarter way. }
 
\label{sec:construction}
To construct automatic contrast sets for GQA
we first identify a large subset of questions requiring specific reasoning skills~(\S\ref{sec:question_identification}). 
Using the scene graph representation, we perturb each question in a manner which changes its gold answer (\S\ref{sec:pertubation}). Finally, we validate the automatic process via crowd-sourcing (\S\ref{sec:mturk}).

\subsection{Identifying Recurring Patterns in GQA}
\label{sec:question_identification}
%% XX\roy{change}\yonatan{It depends which set we refer. We use the balanced set which has 943K in train, 132K in valid and some more in test, but the full GQA contains 22M questions. I think we can remove the XX...} 
The questions in the GQA dataset present a diverse set of modelling challenges, as exemplified in Table~\ref{tab:question_templates}, including object identification and grounding, spatial reasoning and color identification. 
Following the contrast set approach, we create perturbations testing whether models are capable of solving questions which require this skill set, but that diverge from their training distribution.

To achieve this, we identify commonly recurring question templates which specifically require such skills. For example, to answer the question ``\textit{Are there any cats near the boat}?'' a  model needs to identify objects in the image (\textit{cats}, \textit{boat}), link them to the question, and identify their relative position.

We identify six question templates, testing various skills (Table~\ref{tab:question_templates}).
%\yonatan{Last column problem: The numbers in Train and Valid refer to 1 max aug. Maybe we can delete this column? This information is available in the other tables [valid \& train] }. 
We abstract each question template with a regular expression which identifies the question types as well as the physical objects, their attributes (e.g., colors), and spatial relations. Overall, these regular expressions match 29K questions in the validation set ($\approx$22\%)\resolved{\roy{use $\approx$ rather than $\sim$}}, and 80K questions in the training set ($\approx$8\%).

\subsection{Perturbing Questions with Scene Graphs}
\label{sec:pertubation}
We design a perturbation method which guarantees a change in the gold answer for each question template. For example, looking at Fig.~\ref{fig:more_examples}, for the question template \emph{are there \textbf{\textit{X}} near the \textit{Y}?} (e.g., ``Is there any fence near the players?''), we replace either X or Y with a probable distractor (e.g.,\resolved{\roy{no need for italics when writing e.g.}}, replace ``fence'' with ``trees'').

We use the scene graph to ensure that the answer to the question is indeed changed. In our example, this would entail grounding ``players'' in the question to the scene graph (either via exact match or several other heuristics such as hard-coded lists of synonyms or co-hyponyms), locating its neighbors, and verifying that none of them are ``trees.''
%\gabi{Yoantan, how did you deal with actually linking the text ``boat'' to elements in the graph? or is that grounding part of the gqa dataset?}
%% ME: @@ We probably should expand on this - let's check room
%\yonatan{I have a distribution of objects from the scene graphs. So I search intersection (text similarity, or hard-coded synonyms) between the 'boat' in the question to the scene graph distribution. For each (question, answer, image, scene graph) , there is a process to receive a distribution of things that *are not* in the current scene graph. }
We then apply heuristics to fix syntax (e.g., changing from singular to plural determiner, see Appendix~\ref{sec:ling_heuristics}), \resolved{Table~\ref{tab:linguistic_rules}\roy{please point to the appendix section, not the specific table number})} and verify that the perturbed sample does not already exist in GQA.
The specific perturbation is performed per question template. 
In question templates with two objects (\textit{X} and \textit{Y}), we replace \textit{X} with \textit{X'}, such that \textit{X'} is correlated with \textit{Y} in other GQA scene graphs.
In question templates with a single object \textit{X}, we replace \textit{X} with a textually-similar \textit{X'}. For example in the first row in Table~\ref{tab:question_templates} we replace \textit{dishwasher} with \textit{dishes}. Our perturbation code is publicly available.

This process may yield an arbitrarily large number of contrasting samples per question, as there are many candidates for replacing objects participating in questions. We report experiments with up to 1, 3 and 5 contrasting samples per question.

\paragraph{Illustrating the perturbation process.} Looking at Fig.~\ref{fig:perturbed-example}, we see the scene-graph information: \emph{objects} have bounding-boxes around them in the image (e.g., \emph{zebra}); \emph{Objects} have \emph{attributes} (\emph{wood} is an attribute of the \emph{fence} object); and there are \emph{relationships} between the objects (the puddle is to the \textit{right} of the zebra, and it is \emph{near} the fence). The original (question, answer) pair is (``is there  a fence near the puddle?'', ``Yes''). We first identify the question template by regular expressions: ``Is there X near the Y'', and isolate X=\emph{fence}, Y=\emph{puddle}. The answer is ``Yes'', so we know that X is indeed near Y. We then use the existing information given in the scene-graph. We search for X' that is not near Y. To achieve this, we sample a random object (\textit{wall}), and verify that it doesn't exist in the set of scene-graph objects. This results in a perturbed example ``Is there a \emph{wall} near the {puddle}?'', and now the ground truth is computed to be ``No''.\resolved{\michael{Changed `deterministically determined` by compute - I left deterministic in the following paragraph}\roy{A question that reviewers asked and is still unanswered is whether this is done manually or automatically. Can we add a statement such as ``this process is done entirely automatically?'' would that be accurate?}} Consider a different example: (``Is the puddle to the left of the zebra?'', ``Yes''). We identify the question template ``Is the X \textit{Rel} the Y'', where X=\emph{puddle}, Rel=\emph{to the left}, Y=\emph{zebra}. The answer is ``Yes''. Now we can easily change Rel'=\emph{to the right}, resulting in the (question, answer) pair (``Is the puddle to the right of the zebra?'', ``No''). 

\begin{figure*}
\centering
\begin{minipage}{0.3\textwidth}
\includegraphics[width=\textwidth]{images/example_baseball.jpg}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\centering
\captionsetup{type=table} %% tell latex to change to table
\scalebox{0.65}{
\begin{tabular}{@{}ll@{}}

%\multicolumn{1}{c}{\textbf{Examples}}         \\ \midrule
The \textbf{\textit{bat the batter is holding}} has what color? Brown  $\rightarrow$\\ The \textbf{\textit{helmet}} has what color? Blue                      \\ \midrule
Is there any \textbf{\textit{fence}} near the \textit{players}? Yes $\rightarrow$\\ Are there any \textbf{\textit{trees}} near the \textit{players}? No \\ \midrule
Do you see either \textbf{\textit{bakers}} or \textit{photographers}? No        $\rightarrow$\\ Do you see either \textbf{\textit{spectators}} or \textit{photographers}? Yes   \\ \midrule
Is the \textit{catcher} to the \textit{right} of an \textbf{\textit{umpire}}? No         $\rightarrow$\\ Is the \textit{catcher} to the \textit{right} of a \textbf{\textit{batter}}? Yes         \\ \midrule
Is the \textit{catcher} to the \textbf{\textit{right}} of an \textit{umpire}? No         $\rightarrow$\\ Is the catcher to the \textbf{\textit{left}} of an \textit{umpire}? Yes         \\ %\bottomrule
\end{tabular}
}
\end{minipage}
\caption{GQA image (left) with example perturbations for different question templates (right). Each perturbation aims to change the label in a predetermined manner, e.g., from ``yes'' to ``no''.}
\label{fig:more_examples}
\end{figure*}


We highlight the following: (1) This process is done entirely automatically (we validate it in Section~\ref{sec:mturk}); (2) The answer is deterministic given the information in the scene-graph; (3) We do not produce unanswerable questions. If we couldn't find an alternative atom for which the presuppositions hold, we do not create the perturbed (question, answer) pair; (4) Grounding objects from the question to the scene-graph can be tricky. It can involve exact match, number match (\emph{dogs} in the question, and \emph{dog} in the scene-graph), hyponyms (\emph{animal} in the question, and \emph{dog} in the scene-graph), and synonyms (\emph{motorbike} in the question, and \emph{motorcycle} in the scene-graph). The details are in the published code; (5) The only difference between the original and the perturbed instance is a single atom: an object, relationship, or attribute. 

\subsection{Validating Perturbed Instances}
\label{sec:mturk}
To verify the correctness of our automatic process, we sampled 553 images, each one with an original and perturbed QA pair for a total of 1,106 instances ($\approx$4\% of the validation contrast pairs)\resolved{\roy{$\approx$}}. The (image, question) pairs were answered independently by human annotators on Amazon Mechanical Turk (see Fig.~\ref{fig:amt_example} in Appendix~\ref{app:example}), oblivious to whether the question originated from GQA or from our automatic contrast set.
We found that the workers were able to correctly answer 72.3\% of the perturbed questions, slightly lower than their performance on the original questions (76.6\%).\footnote{The GQA paper reports higher human accuracy (around 90\%) on their original questions. We attribute this difference to the selection of a subset of questions that match our templates, which are potentially more ambiguous than average GQA questions (see Section~\ref{sec:experiments}).} 
We observed high agreement between annotators ($\kappa = 0.679$). 

Our analysis shows that the human performance difference between the perturbed questions and the original questions can be attributed  to the scene graph annotation errors in the GQA dataset: 3.5\% of the 4\% difference is caused by a discrepancy between image and scene graph (objects appearing in the image and not in the graph, and vice versa). Examples are available in Fig.~\ref{fig:scene_graph_mistakes} in Appendix~\ref{sec:examples}.

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/03_experiments.tex <==
\label{sec:experiments}

We experiment with two top-performing GQA models, MAC~\cite{arad2018compositional} and LXMERT~\cite{tan-bansal-2019-lxmert},\footnote{MAC and LXMERT are the top two models in the \href{https://eval.ai/web/challenges/challenge-page/225/leaderboard/733}{GQA leaderboard} with a public implementation as of the time of submission: \url{https://github.com/airsplay/lxmert} and  \url{https://github.com/stanfordnlp/mac-network/}. \resolved{\roy{Please add a date, or a statement such as. this will most probably not be true forever, and perhaps not even true now}\yonatan{"As of the time of submission" added. Is it ok?}}} to test  their generalization on our automatic contrast sets, leading to various key observations.


%\roy{don't start with your results. you need to start by describing the rational behind our experiments, then move to the experimental setup, and then discuss our results.}Our results are summarized in Table~\ref{tab:training_improvement}.
%In line with other works on contrast sets, we use our contrast sets to evaluate model performance during inference, showing that top-performing models indeed struggle on the perturbed validation data. 
%In addition, our large scale automatic perturbation process enables us to test its effect during training as well, showing that training on automatic training set perturbation lead to more robust models. \roy{I would start by the first part, we have not discussed the training augmentation part yet and it deserves more than one line intro here}
%In the following we make several interesting observations based on these results.\roy{drop this sentence, it doesn't say anything}

\paragraph{Models struggle with our contrast set.}
% \yonatan{Those tables refers to 1 augmentation per instance, do we want more?}
Table~\ref{tab:training_improvement} 
%\yonatan{The augmented column now describes the Max. 5 augmentation set.} 
shows that despite GQA's emphasis on dataset balance and compositionality, both MAC and LXMERT degraded on the contrast set: MAC 64.9\% $\rightarrow$ 51.5\% and LXMERT 83.9\% $\rightarrow$ 67.2\%, compared to only 4\% degradation in human performance.
Full breakdown of the results by template is shown in  Table~\ref{tab:results_single_augmentation}. 
As expected, question templates that reference two objects ($X$ and $Y$) result in larger performance drop compared to those containing a single object ($X$).
%In general, for more complex or compositional  questions, the perturbation we introduce are less noticeable, but it still changes the answer. 
Questions about colors had the \emph{smallest} performance drop, potentially because the models performance on such multi-class, subjective questions is relatively low to begin with.
% , potentially due to the multi-label\yonatan{I think it's multi-class, not multi-label} nature of these questions, and the ambiguity caused by the similarity between colors such as grey and black, or red and orange. 

\paragraph{Training on perturbed set leads to more robust models.}
Previous works tried to mitigate spurious datasets biases by explicitly balancing labels during dataset construction \cite{goyal2017making,zhu2016visual7w, zhang2016yin} or using adversarial filtering \cite{zellers-etal-2018-swag,zellers-etal-2019-hellaswag}.
In this work we take an inoculation approach \cite{liu-etal-2019-inoculation} and augment the original GQA training set with contrast training data, resulting in a total of 1,023,607 training samples.
We retrain both models on the augmented training data, and observe in Table~\ref{tab:training_improvement}  that their performance on the \emph{contrast set} almost matches that of the original validation set, with no loss (MAC) or only minor loss (LXMERT) to original validation accuracy.\footnote{To verify that this is not the result of training on more data, we repeated this experiment, removing the same amount of original training instances (so the final dataset size is the same as the original one), and observed very similar results.}
%\yonatan{Added footnote - LXMERT re-pretrained without GQA} on the original validation question set. @@ME: Moved to appendix
These results indicate that the perturbed \emph{training} set is a valuable signal, which helps models recognize more patterns.  

\input{figs/breakdown}

\paragraph{Contrast Consistency.}
Our method can be used to generate many augmented questions by simply sampling more items for replacement (Section~\ref{sec:construction}). This allows us to measure the \textit{contrast consistency} \cite{gardner-etal-2020-evaluating} of our contrast set, defined as the percentage of the contrast sets for which a model’s predictions are correct for all examples in the set (including the original example). For example, in Fig.~\ref{fig:perturbed-example} the set size is 4, and only 2/4 predictions are correct. 
We experiment with 1, 3, and 5 augmentations per question with the LXMERT model trained on the original GQA training set. Our results (Table~\ref{tab:consistency}) show that sampling more objects leads to similar accuracy levels for the LXMERT model, indicating that quality of our contrast sets does not depend on the specific selection of replacements. However, we observe that consistency drops fast as the size of the contrast sets per QA instance grows, indicating that model success on a specific instance does not mean it can generalize robustly to perturbations.

\begin{table}[]
\center
\scalebox{0.8}{
\begin{tabular}{cccc}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Augmentations\\per instance\end{tabular}} & \textbf{Contrast sets} & \textbf{Acc.} & \textbf{Consistency} \\ \hline
1                                                                                                      & 11,263                     & 66\%            & 63.4\%               \\
3                                                                                                      & 23,236                     & 67\%            & 51.1\%               \\
5                                                                                                      & 28,968                       & 67\%              & 46.1\%                 \\ \bottomrule
\end{tabular}
}
\caption{Accuracy and consistency results for the LXMERT model on different contrast set sizes.}
\label{tab:consistency}
\end{table}





% The LXMERT model has two stages of training: (1) pre-training on several datasets (including GQA), and (2) fine-tuning on GQA. We perform another experiment with the LXMERT re-pretrained without GQA, and show that we still reach similar improvement on the contrast sets. 

% \subsection{Analysis}
% % COMMENT - I don't think it's very intereseting [yonatan]
% Exploring the initial benchmark (the model trained on the original training set): 
% Out of the tested instances, in 23\% of the cases the model was correct on the original instance, and was wrong on the augmented instance. In 3.8\% of the cases the model was wrong on the original instance, and was correct on the augmented instance. 
% In 0.1\% of the cases the model was wrong on both the original and augmented instance. 

% We ask whether a possible reason for the performance drop, is that the objects that were used in the augmented set are objects that do not occur many times in the training dataset. The model is not familiar enough with such objects after training.

% We performed the following process to check it: (1) Extracting all the augmented (x,y) objects for each question templates. (2) Counting the number of times each (x,y) object appeared in the train set with the same question template. (3) Taking an average of the numbers received in step 2. 
% Simple example to understand this process:
% Question template: ``Do you see X or Y'', $X$=``umbrella'' and $Y$=``car'' appeared 2 times in the training set. 
% Question template: ``Do you see X or Y'', $X$=``sheep'' and $Y$=``man'' appeared 10 times in the training set. 
% The average number of times augmented (x,y) object appeared in the train set is average of 2,10 = 6. The averages received in the end of the process are: for the augmented (x,y) objects, 1.56, and for the original (x,y) objects, 5.44. It means that the original (x,y) objects appeared 3.48 times \textbf{more} than the augmented (x,y) objects. This experiment already answers our hypothesis, but we performed an additional experiment. 

% Next, we partitioned the augmented validation dataset for 3 parts, based on the object occurrences: (1) Low (x,y) objects occurrences (2) Medium (x,y) objects occurrences, and (3) High (x,y) objects occurrences. The \emph{low} partition was taken to be (x,y) objects that did not appear at all in the training dataset. Then, we take the median of the rest of object occurrences. The \emph{medium} partition is objects that occurred below ($\le$) the median, and the \emph{high} partition are objects that occurred above ($>$) the median. We performed it twice, first for the original training dataset, and than to the augmented training dataset (after adding new objects).
% Results are presented at Table~\ref{tab:low_med_high}. In the case of the original dataset, we can see a positive correlation between the occurrences of objects in the training dataset and the performance. This correlation do not seem to exists in the case of the augmented training dataset. 

% \begin{table}[]
% \centering
% \scalebox{0.80}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%                                                                                     &                   & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline
% {\textbf{Train}}                                                     & \textbf{\# Items} & 2,126        & 283             & 244           \\ \cline{2-5} 
%                                                                                     & \textbf{LXMERT}   & 0.65         & 0.71            & 0.78          \\ \cline{2-5} 
%                                                                                     & \textbf{MAC}      & 0.52         & 0.54            & 0.57          \\ \hline
% {\textbf{\begin{tabular}[c]{@{}c@{}}Augmented\\ Train\end{tabular}}} & \textbf{\# Items} & 1,615        & 625             & 413           \\ \cline{2-5} 
%                                                                                     & \textbf{LXMERT}   & 0.84         & 0.84            & 0.83          \\ \cline{2-5} 
%                                                                                     & \textbf{MAC}      & 0.77         & 0.76            & 0.78          \\ \hline
% \end{tabular}
% }
% \caption{Results on the validation set partition by occurrences of (x,y) objects in the training dataset}
% \label{tab:low_med_high}
% \end{table}


==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/05_discussion.tex <==
Our results suggest that both MAC and LXMERT under-perform when tested out of distribution. 
A remaining question is whether this is due to model architecture or dataset design. 
% \citet{gardner2020evaluating} suggests that contrast sets provide a more accurate reflection of  model performance. 
\citet{bogin2020latent} claim that both of these models are prone to fail on compositional generalization because they do not decompose the problem into smaller sub-tasks. Our results support this claim. 
On the other hand, it is possible that  a different dataset could prevent these models from finding shortcuts. Is there a dataset that can prevent \emph{all} shortcuts? 
Our automatic method for creating contrast sets allows us to ask those questions, while we believe that future work in better training mechanisms, as suggested in \citet{bogin2020latent} and  \citet{jin-etal-2020-visually}, could help in making more robust models. 
%An additional hypothesis is that we introduce atoms that are less familiar to the model with training\footnote{We tested the hypothesis and discovered that an original (x,y) pair has appeared 3.5 times more than augmented (x,y) pair in the training dataset}. 

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/06_conclusions.tex <==
We proposed an automatic method for creating contrast sets for VQA datasets that use annotated scene graphs.
We created contrast sets for the GQA dataset, which is designed to be compositional, balanced, and robust against statistical biases. We observed a large performance drop between the original and augmented sets. As our contrast sets can be generated cheaply, we further augmented the GQA training data with additional perturbed questions, and showed that this improves models' performance on the contrast set. Our proposed method can be extended to other VQA datasets.% A full explanation of our empirical observations remains to be found.
% COMMENT - I also want to say, "We conclude that (1) The GQA is good, (2) The performance drop still raises questions 

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/07_acks.tex <==
We thank the reviewers for the helpful comments and feedback.
We thank the authors of GQA for building the dataset, and the authors of LXMERT and MAC for sharing their code and making it usable. This work was supported in part by the Center for Interdisciplinary Data Science Research at the Hebrew University of Jerusalem, and research gifts from the Allen Institute for AI.

==> NAACL - Automatic Generation of Contrast Sets from Scene Graphs/sections/08_ethical_considerations.tex <==

\resolved{\roy{Add some context: we built a dataset, automatically, not requiring manual labor, the goal of our dataset is to improve model robustness against variosu biases. Our dataset is built on the GQA dataset.
Then discuss the annotation part, saying this was the only manual work done on the dataset.}}
We created contrast sets automatically, and verified their correctness via the crowdsourcing annotation of a sample of roughly 1K instances. Section~\ref{sec:mturk} describes the annotation process on Amazon Mechanical Turk. The images and original questions were sampled from the public GQA dataset \cite{hudson2019gqa}, in the English language. Fig.~\ref{fig:amt_example} in Appendix~\ref{app:example} provides example of the annotation task. Overall, the crowdsourcing task resulted in  $\approx$6\ \resolved{roy{approx}} hours of work, which paid an average of 11USD per hour per annotator. \resolved{\roy{do you have an estimate on how much time it took them? i.e., how many hours did it take them to make \$55?}}


